Auditing Visualizations: Transparency Methods Struggle to Detect Anomalous Behavior

Model visualizations provide information that outputs alone might miss. But can we trust that model visualizations reflect model behavior? For instance, can they diagnose abnormal behavior such as planted backdoors or overregularization? To evaluate visualization methods, we test whether they assign different visualizations to anomalously trained models and normal models. We find that while existing methods can detect models with starkly anomalous behavior, they struggle to identify more subtle anomalies. Moreover, they often fail to recognize the inputs that induce anomalous behavior, e.g. images containing a spurious cue. These results reveal blind spots and limitations of some popular model visualizations. By introducing a novel evaluation framework for visualizations, our work paves the way for developing more reliable model transparency methods in the future.

==> localization_table.tex <==
\begin{table*}[t]
    \caption{Localization AUROC for every anomaly and transparency method. We find that all three methods are about as good as chance at localization. \red{Rotate this for better use of space.}}
    \label{localization_res}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{tabular}{lc|cccr}
    \toprule
    Anomaly type & Anomaly & Caricature & Guided Backpropagation & Integrated Gradients \\
    \midrule
    Backdoor & $0$ & 0.5439 & 0.3425 & 0.4850  \\
    & $1$ & 0.4761 & 0.4475 & 0.5550  \\
    & $2$ & 0.5318 & 0.4725 & 0.6475  \\
    & $3$ & 0.4796 & 0.7350 & 0.4975  \\
    & $4$ & 0.5168 & 0.3650 & 0.4550  \\
    & $5$ & 0.4393 & 0.3000 & 0.5850  \\
    Spurious Features & $\delta = 1.0$ & 0.3907 & 0.7050 & 0.3050  \\
    & $\delta = 0.5$ & 0.4700 & 0.3675 & 0.7100  \\
    & $\delta = 0.3$ & 0.5136 & 0.6425 & 0.4300  \\
    & $\delta = 0.1$ & 0.5732 & 0.6400 & 0.2075  \\
    Missing Class &  414 & 0.4904 & 0.3375 & 0.4200  \\
     &  400 & 0.4932 & 0.4050 & 0.5700  \\
     &  218 & 0.4975 & 0.5575 & 0.3850  \\
    Blur & & 0.5704 & 0.5500 & 0.4100  \\
    \bottomrule
    Mean & & {0.499} & 0.491 & 0.476  \\
    \bottomrule
    \end{tabular}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table*}


==> tables/localization/loc_alex.tex <==
\begin{tabular}{lllllllllllllll}
    \toprule
    Anomaly Type & \multicolumn{6}{c}{Backdoor} & \multicolumn{3}{c}{Missing class} & \multicolumn{4}{c}{Spurious}  & Blur \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-10} \cmidrule(lr){11-14}
Anomaly &   0 &   1 &   2 &   3 &   4 &   5 & 218 & 400 & 414 & 0.1 & 0.3 & 0.5 & 1.0 & \ \\
\midrule
GBP                &  \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} &  0.69 &  0.43 &  0.58 &  \textbf{\textbf{0.72}} &  \textbf{\textbf{0.77}} &  \textbf{\textbf{0.80}} &  0.69 & \textbf{\textbf{0.87}} \\
IntGrad            &  \textbf{0.99} & \textbf{0.97} & \textbf{0.98} & \textbf{0.98} & \textbf{0.99} & \textbf{0.94} &  0.57 &  0.61 &  0.46 &  \textbf{\textbf{0.82}} &  \textbf{\textbf{0.77}} &  \textbf{\textbf{0.85}} &  0.42 & \textbf{\textbf{0.85}} \\
Grad-CAM            &  \textbf{0.98} & \textbf{0.99} & \textbf{0.95} & \textbf{0.98} & \textbf{0.99} & \textbf{0.97} &  \textbf{\textbf{0.81}} &  0.58 &  0.59 &  0.53 &  0.55 &  0.53 &  0.53 & \textbf{\textbf{0.76}} \\
Guided Grad-CAM     &  \textbf{0.99} & \textbf{1.00} & \textbf{0.96} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} &  \textbf{\textbf{0.74}} &  0.40 &  0.58 &  0.51 &  0.70 &  0.64 &  0.57 &  \textbf{\textbf{0.79}} \\
{Car}$_{(2,2,1)}$ &  0.37 & 0.40 &  0.50 & 0.45 & 0.52 & 0.50 &  0.38 &  0.45 &  0.67 &  0.57 &  0.48 &  0.57 &  0.52 &  0.28 \\
{Car}$_{(3,0,3)}$ &  0.47 & 0.54 &  0.54 & 0.53 & 0.51 & 0.60 &  0.62 &  0.52 &  0.51 &  0.49 &  0.54 &  0.40 &  0.51 &  0.65 \\
{Car}$_{(3,2,2)}$ &  0.56 &   0.53 &   0.56 &   0.52 &   0.55 &   0.50 &  0.60 &  0.61 &  0.41 &  0.50 &  0.52 &  0.51 &  0.49 &  0.66 \\
{Car}$_{(3,3)}$       &  0.51 &   0.56 &   0.59 &   0.60 &   \textbf{0.71} &   0.68 &  0.56 &  0.47 &  0.62 &  0.57 &  0.55 &  0.46 &  0.53 & \textbf{\textbf{0.82}}\\
{Car}$_{(3,4,3)}$ &  0.57 &   0.59 &   0.53 &   0.58 &   \textbf{0.71} &   0.63 &   0.53 &  0.58 &  0.57 &  0.42 &  0.43 &  0.46 &  0.39 & 0.53 \\
{Car}$_{(4,0,3)}$ &  0.64 &   \textbf{0.80} &   0.67 &   0.48 &   \textbf{0.77} &   \textbf{0.72} &   0.66 &  0.32 &  0.46 &  0.52 &  0.54 &  0.46 &  \textbf{\textbf{0.77}} & 0.59 \\
{Car}$_{(4,2,3)}$ &  \textbf{0.84} &   \textbf{0.91} &   \textbf{0.91} &   \textbf{0.93} &   \textbf{0.81} &   0.69 &   0.51 &  0.46 &  0.50 &  0.55 &  0.51 &  0.52 &  0.64 & \textbf{\textbf{0.73}}\\
\bottomrule
\end{tabular}


